Gradual C0: Symbolic Execution for Gradual Verification

Current static verification techniques support a wide range of programs. However, such techniques only support complete and detailed specifications, which places an undue burden on users. To solve this problem, prior work proposed gradual verification, which handles complete, partial, or missing specifications by soundly combining static and dynamic checking. Gradual verification has also been extended to programs that manipulate recursive, mutable data structures on the heap. Unfortunately, this extension does not reward users with decreased dynamic checking as specifications are refined. In fact, all properties are checked dynamically regardless of any static guarantees. Additionally, no full-fledged implementation of gradual verification exists so far, which prevents studying its performance and applicability in practice. We present Gradual C0, the first practicable gradual verifier for recursive heap data structures, which targets C0, a safe subset of C designed for education. Static verifiers supporting separation logic or implicit dynamic frames use symbolic execution for reasoning; so Gradual C0, which extends one such verifier, adopts symbolic execution at its core instead of the weakest liberal precondition approach used in prior work. Our approach addresses technical challenges related to symbolic execution with imprecise specifications, heap ownership, and branching in both program statements and specification formulas. We also deal with challenges related to minimizing insertion of dynamic checks and extensibility to other programming languages beyond C0. Finally, we provide the first empirical performance evaluation of a gradual verifier, and found that on average, Gradual C0 decreases run-time overhead between 11-34% compared to the fully-dynamic approach used in prior work. Further, the worst-case scenarios for performance are predictable and avoidable.

==> contents/insertlast-sv-table.tex <==


\begin{tabular}{|p{0.13\linewidth} | p{0.3\linewidth} | p{0.3\linewidth} | p{0.15\linewidth} |}
\hline
\multicolumn{2}{|c|}{\textbf{Specification Increment}} & \multicolumn{2}{c|}{\textbf{Verifier Output}} \\ \hline
\textbf{Lines from \fig\ref{fig:ll-insert-sv}} & \multicolumn{1}{c|}{\textbf{Content}} &  \multicolumn{1}{c|}{\textbf{Viper}} & \multicolumn{1}{c|}{\textbf{\gco}} \\ \hline\hline
    & precondition, postcondition, \ttt{acyclic}, \ttt{acyclicSeg} 
      \newline \gco has $\qm$ on loop invariant & While statement might fail. There might be insufficient permission to access y.next 
    & success \\ \hline
    & last increment + loop invariant $\phiAcc{\ttt{y->next}}$ 
      \newline \gco has $\qm$ on loop invariant and precondition
    & Loop invariant might not hold on entry. There might be insufficient permission to access y.next 
    & success \\ \hline
    & last increment + unfolds of acyclic and acyclicSeg
      \newline \gco has $\qm$ on loop invariant
    & Loop invariant might not be preserved. There might be insufficient permission to access y.next.
    & success \\ \hline
    & last increment + unfold acyclicSeg(y,NULL) + $\phiAnd \phiAcc{\ttt{y->val}}$ $\phiAnd \ttt{acyclicSeg(y->next,NULL)}$ in loop invariant
      \newline \gco has $\qm$ on loop invariant
    & Postcondition of insertLast might not hold. There might be insufficient permission to access acyclic(list).
    & success \\ \hline
    & last increment + folds for end of list, fold for acyclic(list)
      \newline \gco has $\qm$ on
    & Folding acyclic(list) might fail. There might be insufficient permission to access acyclicSeg(list, null).
    & \\ \hline
    & last increment + acyclicSeg(list,y) in loop invariant
      \newline \gco has $\qm$ on 
    & Loop invariant might not hold on entry. There might be insufficient permission to access acyclicSeg(list, y).
    & \\ \hline
    & last increment + fold acyclicSeg(list,y)
      \newline \gco has $\qm$ on 
    & Loop invariant might not be preserved. There might be insufficient permission to access acyclicSeg(list, y).
    & \\ \hline
    & last increment + folds in loop body
      \newline \gco has $\qm$ on 
    & Loop invariant might not be preserved. There might be insufficient permission to access acyclicSeg(list, y).
    & \\ \hline
    & last increment + mergeLemma in loop body + mergeLemma in for acyclic
      \newline \gco has $\qm$ on 
    & success
    & \\ \hline
\end{tabular}

% notes about increment
% - want to know that acyclic + acyclicSeg + pre/post is correct
% - need a while loop providing permission to y->next on every iteration of the loop, so write loop invariant that exposes that for the current node y->next
% - need to hold on entry to the loop so unfold acyclic + acyclicSeg for this information
% - realize that acc(y->next) needs to hold on every iteration of the loop which means we need permission to all heap locations in the list the while loop is iterating over, so we really need a stronger invariant and to unroll acyclicSeg(y->next, NULL) on every iteration to; need to have permission to first node and rest of nodes in list 
% work on what we need for acyclic(list); need acyclicSeg(list,null), which means we need acc(list->next) && acc(list->val) && acyclicSeg(list->next, null); so we have to build up bottom up that the list is acyclic; look at what we can get from the statements after the loop; the new end of the list is acyclic, but can't build up further from this at this point; we need this to come from the loop invariant: missing the list up to that point is acyclic, which can only come from the loop invariant; strengthen it with acyclicSeg(list,y)
% but our specification isn't set up for this to hold on entry and so we add the fold on line 57
% and then it is also not preserved by the loop invariant, so spend time thinking about how to fold back up the the permissions exposed at every iteration of the loop
% however folding up the permissions is not enough, need a lemma to prove transitivity because, having acyclic(list, tmp) and acyclic(tmp,y) is not the same as having acyclic(list,y); realize the same is needed for acyclic(list) + be done


% \begin{table}[t]
% {\small
% \centering
% \input{contents/insertlast-sv-table}}

% \disableTttResize
% \captionsetup{font=footnotesize}
% \caption[font=footnotesize]{TBD}
% \label{tbl:insertlast-incremental}
% \vspace{-1.5em}
% \end{table}


==> contents/table_vs_dynamic.tex <==

\scriptsize
\begin{tabular}{l|c|cccc|cccc|c|}
\cline{2-11}
\multirow{2}{*}{\textbf{Example}}                        & \multirow{2}{*}{\textbf{$\omega$}} & \multicolumn{4}{c|}{\textbf{\% $\Delta t$, GV vs. DV}}                                            & \multicolumn{4}{c|}{\textbf{\% Steps GV<DV  for Paths DV < GV}}           & \multirow{2}{*}{\textbf{\% Paths GV < DV}} \\ \cline{3-10}
                                                         &                                    & \multicolumn{1}{c|}{\textit{Mean}}  & \multicolumn{1}{c|}{\textit{St. Dev.}} & \multicolumn{1}{c|}{\textit{Max}}   & Min  & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{St. Dev.}} & \multicolumn{1}{c|}{\textit{Max}}  & \textit{Min.} &                                                   \\ \hline\hline
\multicolumn{1}{c|}{\multirow{3}{*}{Binary Search Tree}} & 16                                 & \multicolumn{1}{c|}{-60.5} & \multicolumn{1}{c|}{20.1}     & \multicolumn{1}{c|}{-89.9} & 30.2 & \multicolumn{1}{c|}{98.4} & \multicolumn{1}{c|}{1.9}      & \multicolumn{1}{c|}{100}  & 1.9  & 25.8                                              \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                    & 32                                 & \multicolumn{1}{c|}{-73.6} & \multicolumn{1}{c|}{22.0}     & \multicolumn{1}{c|}{-95.4} & 16.4 & \multicolumn{1}{c|}{98.8} & \multicolumn{1}{c|}{1.6}      & \multicolumn{1}{c|}{100}  & 1.6  & 35.5                                              \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                    & 64                                 & \multicolumn{1}{c|}{-79.3} & \multicolumn{1}{c|}{23.4}     & \multicolumn{1}{c|}{-98.7} & 7.6  & \multicolumn{1}{c|}{99.1} & \multicolumn{1}{c|}{1.4}      & \multicolumn{1}{c|}{100}  & 1.4  & 51.6                                              \\ \hline
\multirow{3}{*}{Linked List}                             & 32                                 & \multicolumn{1}{c|}{-51.9} & \multicolumn{1}{c|}{39.0}     & \multicolumn{1}{c|}{-88.5} & 26.5 & \multicolumn{1}{c|}{79.8} & \multicolumn{1}{c|}{14.4}     & \multicolumn{1}{c|}{98.8} & 14.4 & 0                                                 \\ \cline{2-11} 
                                                         & 64                                 & \multicolumn{1}{c|}{-59.6} & \multicolumn{1}{c|}{45.4}     & \multicolumn{1}{c|}{-96.5} & 19.3 & \multicolumn{1}{c|}{72.5} & \multicolumn{1}{c|}{18.7}     & \multicolumn{1}{c|}{98.8} & 18.7 & 0                                                 \\ \cline{2-11} 
                                                         & 128                                & \multicolumn{1}{c|}{-62.3} & \multicolumn{1}{c|}{46.7}     & \multicolumn{1}{c|}{-98.7} & 17.2 & \multicolumn{1}{c|}{69.6} & \multicolumn{1}{c|}{19.7}     & \multicolumn{1}{c|}{98.8} & 19.7 & 0                                                 \\ \hline
\multirow{3}{*}{Composite}                               & 8                                  & \multicolumn{1}{c|}{-78.8} & \multicolumn{1}{c|}{19.7}     & \multicolumn{1}{c|}{-96.5} & 13.2 & \multicolumn{1}{c|}{99.2} & \multicolumn{1}{c|}{0.9}      & \multicolumn{1}{c|}{96.9} & 0.9  & 48.4                                              \\ \cline{2-11} 
                                                         & 16                                 & \multicolumn{1}{c|}{-88.3} & \multicolumn{1}{c|}{19.7}     & \multicolumn{1}{c|}{-99.2} & 11.8 & \multicolumn{1}{c|}{98.4} & \multicolumn{1}{c|}{1.9}      & \multicolumn{1}{c|}{93.7} & 1.9  & 41.9                                              \\ \cline{2-11} 
                                                         & 32                                 & \multicolumn{1}{c|}{-91.4} & \multicolumn{1}{c|}{19.9}     & \multicolumn{1}{c|}{-99.8} & 10.4 & \multicolumn{1}{c|}{98.1} & \multicolumn{1}{c|}{2.2}      & \multicolumn{1}{c|}{92.1} & 2.2  & 35.5                                              \\ \cline{2-11} 
\end{tabular}


==> contents/vcs_excluded.tex <==
\subsubsection{Verification Conditions} A \textit{verification condition} (VC) is a single conjunctive term of a specification that is asserted during verification. \gviper records the total VCs for a spec, denoted $VC_T$, as well the number that were statically eliminated, $VC_S$. The remainder, $VC_T - VC_S$, is checked at run-time. Figure \ref{fig:vcs} shows the average values of $VC_S$ and $VC_T$ across all paths at each step.

We observe that, in absolute numbers, the answer to \textbf{RQ1} is yes: the number of specifications verified statically increases in all three benchmarks as specifications are added to the program.  The gap between static and dynamically-verified specifications does grow in absolute and in relative terms, though.  Note that due to the limitation in our tool mentioned earlier, the ending point is with complete specifications that are nevertheless imprecise (include a ?).  All three programs verify statically, so removing all of the imprecision from the final programs does reduce this gap to zero (no dynamic checks).

As such, with our current configuration, the answer to \textbf{RQ1} is no, but this is highly conditional on our approach to leave each specification imprecise and to remove Boolean literals. Preserving literals and removing imprecision once possible would lead to a decrease in VCs due to eliminating run-time checks that occur purely to support the soundness of our approach, and are dependent on the presence or absence of precision.

When an imprecise predicate body is folded, all permissions are dropped, since the verifier cannot determine if more permissions are required than what the static component of the predicate's body provides. Similarly, all permissions are lost at the boundary of a precise method call, inducing runtime checks to restore them once the function returns. In each case, run-time checks will be added, regardless of the completeness of a specification. 

\begin{figure}
    \centering
\includegraphics[width=.32\textwidth]{figures/vcs_bst.pdf}\hfill
\includegraphics[width=.32\textwidth]{figures/vcs_list.pdf}\hfill
        \includegraphics[width=.32\textwidth]{figures/vcs_composite.pdf}\\
    \vspace{1em}
    \scriptsize
    \cbox{legend_green} $VC_T$ \quad \cbox{legend_purple} $VC_S$\quad
    \cbox{legend_green_light}\ / \cbox{legend_purple_light} Standard Deviation

    \caption{For each example, the average quantity of verification conditions ($VC_T$) and the subset that were eliminated statically ($VC_S$) at each level of completeness across all paths sampled. Shading indicates the standard deviation for counts of each category of VC.}\hfill
    \label{fig:vcs}
\end{figure}

